Parallel Distributional Deep Reinforcement Learning for Mapless Navigation of Terrestrial Mobile Robots

This paper introduces novel deep reinforcement learning (Deep-RL) techniques using parallel distributional actor-critic networks for navigating terrestrial mobile robots. Our approaches use laser range findings, relative distance, and angle to the target to guide the robot. We trained agents in the Gazebo simulator and deployed them in real scenarios. Results show that parallel distributional Deep-RL algorithms enhance decision-making and outperform non-distributional and behavior-based approaches in navigation and spatial generalization.

==> sections/abs.tex <==
\abstract{
Kolmogorov-Arnold Networks (KANs) have shown potential as an alternative to Multi-Layer Perceptrons (MLPs) in neural networks, providing universal function approximation with fewer parameters and reduced memory usage. In this paper, we explore the use of KANs as function approximators within the Proximal Policy Optimization (PPO) algorithm. We evaluate this approach by comparing its performance to the original MLP-based PPO using the DeepMind Control Proprio Robotics benchmark. Our results indicate that the KAN-based reinforcement learning algorithm can achieve comparable performance to its MLP-based counterpart, often with fewer parameters. These findings suggest that KANs may offer a more efficient option for reinforcement learning models. Our implementations can be found in the following link: \url{https://github.com/victorkich/Kolmogorov-PPO}.
}

\keywords{Deep Reinforcement Learning, Robotics, Kolmogorov-Arnold Networks}



==> sections/ack.tex <==
\section*{ACKNOWLEDGEMENT}

This work was supported by the Ministry of Education, Culture, Sports, Science and Technology (MEXT) scholarship. We are also grateful for the support provided by the Human-Centered AI program at the University of Tsukuba.


==> sections/conclusion.tex <==
% \section{Conclusion}\label{conclusion}

% In our evaluation of 1000 steps on the HalfCheetah environment, we observed that the Multi-Layer Perceptron (MLP) with 2 hidden layers of 64 units completed the task significantly faster, with an average elapsed time of 0.37 seconds, compared to the Kolmogorov-Arnold Network (KAN) with no hidden layers (k=2, g=3), which took in average 3.39 seconds. Despite the KAN having far fewer parameters, its increased computational complexity arises from the use of B-splines as activation functions, which require more intricate calculations. The MLP's architecture, while parameter-heavy, benefits from highly optimized implementations in libraries such as Torch, resulting in faster execution times. As KANs are relatively novel, there is a lack of specialized optimization techniques and frameworks designed specifically for them. This discrepancy highlights the potential need for further research and development to enhance the computational efficiency of KANs, making them more viable for real-time applications.

\section{Conclusion}\label{conclusion}

Our study demonstrated that Kolmogorov-Arnold Networks can achieve performance comparable to traditional Multi-Layer Perceptrons with significantly fewer parameters in reinforcement learning tasks. This makes KANs a promising alternative, especially in resource-constrained environments where memory and computational efficiency are critical. However, the current limitations in computational speed due to the complexity of B-spline activation functions suggest the need for further research and optimization. Future work should focus on developing specialized optimization techniques and frameworks for KANs to improve their computational efficiency and make them more suitable for real-time applications.

==> sections/intro.tex <==
\section{Introduction}\label{intro}

Kolmogorov-Arnold Networks (KANs) \cite{liu2024kan} are learnable approximators based on the Kolmogorov-Arnold representation theorem~\cite{kolmogoroff1957representation}, which states that any multivariate continuous function can be expressed as a finite sum of continuous univariate functions. KANs can approximate functions with fewer neurons compared to Multi-Layer Perceptrons (MLPs), thereby reducing network complexity. This simplification enables easier function decomposition, allowing for more straightforward and targeted architecture designs tailored to specific problems. Additionally, KANs utilize less memory and enhance model interpretability, making them highly appealing for various machine learning applications.

Reinforcement Learning (RL)\cite{sutton2018reinforcement} has proven efficient for continuous control tasks such as autonomous robot manipulation\cite{nguyen2019review}, navigation~\cite{zhu2021deep}, and video game playing~\cite{hafner2023mastering}, \cite{wang2023voyager}. Proximal Policy Optimization (PPO)\cite{schulman2017proximal} is a Deep RL algorithm that employs model-free online reinforcement learning to approximate an optimal policy over online training experiences. This algorithm is a cornerstone in the field, excelling in numerous benchmarks and serving as the foundation for newer models like Multi-Agent PPO~\cite{yu2022surprising}, PPO with Covariance Matrix Adaptation~\cite{hamalainen2020ppo}, PPO with Action Mask~\cite{tang2020implementing}, and PPO with Policy Feedback~\cite{gu2021proximal}.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{images/diagram_kan_ppo.pdf}
    \caption{Overview of the proposed framework.}
    \label{fig:curled-dreamer}
    \vspace{-4mm}
\end{figure}

Networks with fewer parameters yet equal or superior approximation capabilities have the potential to significantly enhance performance in various deep reinforcement learning applications. In this work, we propose the use of KANs as policy and value approximators for PPO. The main contributions of this paper are:

\begin{itemize}
\item The first application of KANs as function approximators in a reinforcement learning algorithm.
\item A performance comparison between KAN-based and MLP-based Proximal Policy Optimization in robotics control.
\end{itemize}

The paper is organized as follows: In Section~\ref{related}, we review related works and research in the field. Section~\ref{theoretical} provides the mathematical background of the techniques employed. The proposed methodology is presented in Section~\ref{methodology}. Section~\ref{results} presents the results and evaluation analysis. Finally, we discuss our findings in Section~\ref{conclusion}.

% KAN

% inspired on the kolmogorov arnold represantation theorem that states that any multi variate function can be written as a sum over univariate functions for each variable: y = F(x, z, w) = f (fi1(x) + fi2(z) + fi3(w)), being f and fi's univariate functions and this f can multiple other univariate functions, meaning:
% sum from p = 1 to m over fp(sum from q = 1 to n over fipq(xq)), to represent a multi variable function.

% in machine learning instead of mlp approach:
% price = F(bedrooms, area, age)
% we use:
% price  = f(fi1(bedrooms) + fi2(area) + fi3(age))

% this functions will be processing single inputs, which makes interpratation easier

% more generaly we will have: 
% price  = f(fi1(bedrooms) + fi2(area) + fi3(age)) + f2(fi3(bedrooms) + fi4(area) + fi5(age)) + f3(fi6(bedrooms) + fi7(area) + fi8(age)) + ...

% final formula of the theorem:

% Y = sum from p = 1 to m of function->p(sum from q = 1 to n of function->oq(xq))

% phis will be b splines, the activation functions

% a kan layer will be basically a set of splines which you receive particular inputs like, phi1, phi2 phi3 receive x and the other receive y. and then there will be summs between phi1 and 4, phi 2 and 5 and phi3 and 6. basically there will be an exact number of phis for each input variable, and the sum will be made based on index, the first phi of x with the first phi of y, and so on. the results of the sums of the phis will be used as input values for the next kan layer (phis and sum of results).

% the phis (learnable activation functions) will be all diferentiatiable, meaning we can backpropagate and train parameters. bsplines are piecewise polynomial curves composed of a sequence of lower-order polynomial segments, these polynomial segments are from any order, and will receive the x variable, they are defined by multiple control points to influence the shape of the aproximated polynomial. changing a control point only affects the curve locally which is good, since training samples will afect curves locally and not generaly (which would rearrange the whole polynomium)
% the parameters are the control points

% we will randomly initialize the curves with random parameters, pass the input features, get the final prediction, calculate loss and backpropagate updating the weights for each bspline

% PPO

% Proximal Policy Optimization (PPO) is widely regarded as a strong baseline in the field of deep reinforcement learning (DRL). Since its introduction by OpenAI in 2017, PPO has gained popularity due to its balance of simplicity, ease of implementation, and robust performance across various tasks. While newer and more sophisticated algorithms continue to emerge, PPO remains a standard against which many of these new methods are compared.

% ppo é policy gradient method (online, não usa replay buffer, aprende direto do que o agente ta observando)
% online é normalmente menos sample efficient
% foco em sample efficiency, ease of implementation, stability, low hyparameter tuning


% policy gradient loss standart: (calculada todos os steps) = expectation do log (probabilidades) das ações da política * estimate da advantage function (estimative of the value of the selected action, discounted sum of rewards (calculado ground truth no final do episodio) - baseline estimate (value function, estimativa do retorno dado cada step))

% advantage function -> how good was the action that i took based on what the normal expectation value for that state is. did my action made a better return than expected? positive advantage function means the action returned better than expected and given the loss, the positive value causes the policy to shift towards that action, if advantage function is negative, the policy due to the loss will shift on the other direction (not towards that action)



% to avoid the policy to shift way to much and loose itself (since it is online, the observations are very limited), it includes in the loss function a penality to not go to far from the old policy in an optimization step

% loss = expectation value (new_policy logs /old_policy logs * expectation value)

% shifts towards a better policy but not to much, since it wants policy/old_policy close to one meaning the current action's probability is close to the probability it was in the old policy 

% trpo is the inspiration for that (trust region), loss do not want to go to far from the state region it knows the rewards will be good (trust region)

% ppo loss clip

% E (min(normal policy gradient objective for the current policy * advantage (pushes policy to better (higher) advantage), (same formula but clipped between 1- epsilon and 1 + epslion) * advantage)), epsilon is 0.2 usually

==> sections/methods.tex <==
\section{Methodology}\label{methodology}

We conducted our experiments using six environments from the Gymnasium Mujoco suite, specifically adapted from the DeepMind Control Proprio benchmarks \cite{tassa2018deepmind}. These environments are well-suited for evaluating continuous control tasks and include: HalfCheetah-v4, Hopper-v4, InvertedPendulum-v4, Pusher-v4, Swimmer-v4, and Walker2d-v4. These environments provide a diverse set of challenges, testing the ability of the agent to learn different types of motion and control strategies.

Our implementation utilizes the PPO algorithm as the core reinforcement learning method. PPO is a state-of-the-art algorithm known for its stability and efficiency in policy gradient methods \cite{schulman2017proximal}. We incorporated KANs as the function approximators for both the policy (actor) and value (critic) functions, replacing the traditional MLP used in standard PPO implementations.

\subsection{Network Architectures}

We designed and compared several network architectures for the policy (actor) and value (critic) functions to evaluate the effectiveness of KANs versus MLPs. The configurations included:
\begin{itemize}
\item \textbf{MLP (a=2, c=2)}: Two hidden layers for both actor and critic with 64 units each.
\item \textbf{MLP (a=1, c=2)}: One hidden layer for the actor and two hidden layers for the critic, with 64 units each.
%\item \textbf{MLP (a=1, c=1)}: One hidden layer for both actor and critic, with 64 units each.
\item \textbf{KAN (k=2, g=3)}: KAN for the actor with no hidden layers, order $k=2$ and grid $g=3$, and a critic implemented as an MLP with 2 hidden layers of 64 units each.
\item \textbf{Full KAN (k=2, g=3)}: Both the actor and critic networks implemented using KANs with no hidden layers, order $k=2$ and grid $g=3$.
\end{itemize}

The parameter settings for KANs were chosen based on preliminary tests where we evaluated various configurations to identify the most effective setup. Our tests demonstrated that a KAN with no hidden layers, order $k=2$, and grid $g=3$ provided the best performance in terms of computational efficiency and approximation capability. Consequently, we adopted this architecture for intensive testing.

For the Kolmogorov-Arnold Network, we set the parameters $k=2$ and $g=3$ based on these preliminary findings, ensuring the network's ability to approximate the continuous functions involved in control tasks while maintaining low computational complexity. The number of parameters in the KAN configurations is significantly lower compared to the MLP counterparts, highlighting the efficiency of KANs. The average number of parameters for each configuration across the environments is shown in Table~\ref{params-table}.

\begin{table}[bp]
  \vspace{-4mm}
  \caption{Number of parameters (actor) for different DMC Proprio environments.}
  \label{params-table}
  \centering
  \setlength{\tabcolsep}{4.5pt}
  \begin{tabular}{lrrr}
    \mytoprule
    \textbf{Task} & \textbf{MLP} & \textbf{MLP} & \textbf{KAN} \\
    \textit{Settings} & {\small(a=2, c=2)} & {\small(a=1, c=2)} & {\small(k=2, g=3)} \\
    \mymidrule
    HalfCheetah-v4       & 5702   & 1542    & 510 \\
    Walker2d-v4          & 5702   & 1542    & 510 \\
    Hopper-v4            & 5123   & 963     & 165 \\
    InvertedPendulum-v4  & 4545   & 385     & 20  \\
    Swimmer-v4           & 4866   & 706     & 80  \\
    Pusher-v4            & 6151   & 1991    & 805 \\
    \mymidrule
    \textit{Average of Parameters} & 5348 & 1188 & 348 \\
    \mybottomrule
  \end{tabular}
\end{table}

\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\linewidth]{images/reward_average_plots.pdf}
    \caption{Reward average comparison for all the trained environments using the proposed architectures (using 5 seeds).}
    \label{fig:rewards}
    \vspace{-1mm}
\end{figure*}

\begin{table*}[tbp]
  \caption{DMC Proprio scores for control inputs at 1M train steps. Scores between the top 5\% are shown in bold format.}
  \label{dmc-scores-table}
  \centering
  \setlength{\tabcolsep}{10pt}
  \begin{tabular}{lrrrrr}
    \mytoprule
    \textbf{Task} & {\small\textbf{Full KAN (k=2, g=3)}} & {\small\textbf{KAN (k=2, g=3)}} & {\small\textbf{MLP (a=2, c=2)}} & {\small\textbf{MLP (a=1, c=2)}} \\
    \textit{Train Steps} & 1M & 1M & 1M & 1M \\
    \mymidrule
    HalfCheetah-v4      & 2490   & \textbf{2644}    & 1803   & 1791 \\
    Hopper-v4           & 1633    & \textbf{2031}   & 1897   & 1918 \\
    InvertedPendulum-v4 & 653   & \textbf{818}   & 694   & \textbf{861} \\
    Pusher-v4           & -64  & -52  & \textbf{-39}  & -47 \\
    Swimmer-v4          & 45   & 94   & \textbf{102}   & 82 \\
    Walker2d-v4         & 1487   & 889   & \textbf{3439}   & 2593 \\
    \mymidrule
    \textit{Reward Mean}       & 1358   & \textbf{1540}   & 1482   & 1399 \\
    \textit{Average of Parameters (actor+critic)} &  415  &  5490  &  10490  &  6330 \\
    \mybottomrule
  \end{tabular}
\end{table*}

\subsection{Training Procedure}

Each agent was trained for 1 million steps in each environment. We used the following hyperparameters for training:
\begin{itemize}
    \item \textbf{Number of Environments}: $1$
    \item \textbf{Learning Rate}: $3 \times 10^{-4}$
    \item \textbf{Clip Parameter $\epsilon$}: $0.2$
    \item \textbf{Number of Epochs}: 10
    \item \textbf{Batch Size}: 64
    \item \textbf{Discount Factor $\gamma$}: 0.99
    \item \textbf{GAE Parameter $\lambda$}: 0.95
    \item \textbf{Seeds}: [0, 1, 2, 3, 4]
    \item \textbf{Device}: CPU
\end{itemize}

The agents' performance was evaluated based on the average cumulative reward obtained over 100 evaluation episodes after the training period. The evaluation episodes were conducted without exploration noise to accurately assess the learned policies' effectiveness.


% \subsection{Results Analysis}

% The results were compared using statistical tests to ensure that the observed differences in performance were significant. We performed a t-test on the average returns to compare the KAN-based PPO with the MLP-based PPO. Additionally, we plotted the learning curves to visualize the training process and the stability of the learned policies.

% The experiments demonstrated that the KAN-based PPO generally matched or exceeded the performance of the MLP-based PPO, with a significantly lower number of parameters. This suggests that KANs can provide a more efficient and potentially more interpretable alternative to MLPs in reinforcement learning tasks.


==> sections/related.tex <==
% \section{Related Works}\label{related}

% KANs have recently garnered significant attention for their versatility and enhanced performance across a range of applications. Numerous studies have explored KANs as alternatives to traditional Multilayer Perceptrons (MLPs), consistently demonstrating their superiority in specific scenarios. Concurrently, online reinforcement learning has been a cornerstone in the domain of continuous control tasks, underscoring the importance of investigating KANs' potential in this field. Evaluating whether KANs can compete with or surpass MLPs in reinforcement learning applications is a critical area of exploration. This section reviews pivotal research contributions relevant to this research.

% Developing on the KAN framework, Bozorgasl and Chen~\cite{bozorgasl2024wav} introduced Wav-KAN, a neural network architecture that integrates wavelet functions~\cite{antoniadis1997wavelets} into the KAN framework. This innovation addresses common challenges faced by traditional multilayer perceptrons (MLPs), such as interpretability, training speed, robustness, computational efficiency, and performance. By incorporating wavelet functions, Wav-KAN can effectively capture both high-frequency and low-frequency components of the input data, enhancing overall performance.

% In another significant study, Rubio et al.~\cite{vaca2024kolmogorov} highlighted the effectiveness of KANs in predicting satellite traffic, demonstrating their superiority over traditional MLPs for time series analysis. Similarly, Genet and Hugo~\cite{genet2024tkan} introduced Temporal Kolmogorov-Arnold Networks (TKANs), which combine elements of KANs and Long Short-Term Memory (LSTM) networks. This hybrid architecture improves time series forecasting by leveraging the strengths of both KANs and LSTMs.

% Yang, Qin, and Yu~\cite{yang2024endowing} proposed a novel framework that enhances the interpretability of neural cognitive diagnosis models (CDMs) using KANs while maintaining high accuracy. They introduced two methods: replacing traditional MLPs in existing neural CDMs with KANs, and designing a new aggregation framework entirely based on KANs. This two-level KAN structure processes student, exercise, and concept embeddings at the lower level, and combines these outputs at the upper level for final predictions. Their experimental results on four real-world datasets showed that the KA2NCD framework outperforms traditional and neural CDMs in both accuracy and interpretability, demonstrating its potential in intelligent education systems.


% Online Reinforcement Learning has been succesfully applied multiple times to robotic tasks, it is defined as a method where an agent continuously learns from an ongoing interaction with the environment, rather than learning from a fixed dataset (memory replay). Making use of this paradigm, Zhang, Pang and Hu~\cite{zhang2019trajectory} presented a novel approach to solving the trajectory tracking problem for manipulators and mobile robots using PPO with Generalized Advantage Estimation and Long Short-Term Memory networks as actor and critic. In a similar vein, Lopes et al~\cite{lopes2018intelligent} explored the application of Proximal Policy Optimization to control a quadrotor, which is an inherently unstable aerial platform. The authors demonstrate that the model-free online reinforcement learning algorithm can be effectively used to train a reliable control policy for quadrotor position control.

% In the humanoid robots area, Melo et al~\cite{melo2021learning} succesfully made use of PPO to develop running skills in a humanoid robot, utilizing the RoboCup 3D Soccer Simulation environment, where humanoid robots compete in simulated soccer matches. More on locomotion. Online reinforcement learning had its use expanded between robotics and videogame playing. Proctor~\cite{proctor2021proximal} utilized the algorithm for localizing and searching for lost nuclear sources in a designated area, which is vital for societal safety and reducing human harm. 


% To the best of our knowledge, no efforts in applying KANs as alternatives to mlps is present in the literature, making this a pivotal effort.

\section{Related Works}\label{related}

KANs have recently garnered significant attention for their versatility and enhanced performance across various applications. Numerous studies have explored KANs as alternatives to traditional Multilayer Perceptrons, consistently demonstrating their superiority in specific scenarios. Concurrently, online reinforcement learning has been a cornerstone in the domain of continuous control tasks, underscoring the importance of investigating KANs' potential in this field. Evaluating whether KANs can compete with or surpass MLPs in reinforcement learning applications is a critical area of exploration. This section reviews pivotal research contributions relevant to this research.

Expanding on the KAN framework, Bozorgasl and Chen~\cite{bozorgasl2024wav} introduced Wav-KAN, a neural network architecture that integrates wavelet functions~\cite{antoniadis1997wavelets} into the KAN framework. This innovation addresses common challenges faced by traditional MLPs, such as interpretability, training speed, robustness, computational efficiency, and performance. By incorporating wavelet functions, Wav-KAN effectively captures both high-frequency and low-frequency components of the input data, enhancing overall performance.

Exploring KANs' performance on predicting time series, Rubio et al.~\cite{vaca2024kolmogorov} demonstrated the effectiveness of these networks in predicting satellite traffic, showing their superiority over traditional MLPs for time series analysis. Similarly, Genet and Hugo~\cite{genet2024tkan} introduced Temporal Kolmogorov-Arnold Networks (TKANs), combining elements of KANs and Long Short-Term Memory (LSTM) networks to improve time series forecasting.

Expanding on the exploration of KANs' capabilities, Yang, Qin, and Yu~\cite{yang2024endowing} proposed a novel framework that enhances the interpretability of neural cognitive diagnosis models (CDMs) using KANs while maintaining high accuracy. They introduced two methods: replacing traditional MLPs in existing neural CDMs with KANs and designing a new aggregation framework entirely based on KANs. Their experimental results on four real-world datasets showed that the KA2NCD framework outperforms traditional and neural CDMs in both accuracy and interpretability, demonstrating its potential in intelligent education systems.

Online Reinforcement Learning, where an agent continuously learns from ongoing interaction with the environment, instead of using memory replay, has been successfully applied to various robotic tasks. Zhang, Pang, and Hu~\cite{zhang2019trajectory} presented a novel approach to solving the trajectory tracking problem for manipulators and mobile robots using PPO with Generalized Advantage Estimation and Long Short-Term Memory networks as actor and critic. Similarly, Lopes et al.~\cite{lopes2018intelligent} explored the application of Proximal Policy Optimization to control a quadrotor, demonstrating that model-free online reinforcement learning can effectively train a reliable control policy for quadrotor position control. In the humanoid robots area, Melo et al.~\cite{melo2021learning} successfully utilized PPO to develop running skills in a humanoid robot, using the RoboCup 3D Soccer Simulation environment, where humanoid robots compete in simulated soccer matches. Expanding the use of online reinforcement learning to other areas, Proctor~\cite{proctor2021proximal} used the algorithm for localizing and searching for lost nuclear sources in a designated area, which is vital for societal safety and reducing human harm.

To the best of our knowledge, no efforts have been made to apply KANs as alternatives to MLPs in reinforcement learning, making this study a pivotal contribution.


==> sections/results.tex <==
% \section{Results}\label{results}

% The performance of the KAN-based PPO was evaluated against the MLP-based PPO across the selected environments. The primary metrics considered were the average return and the number of parameters. The goal was to assess whether KANs can achieve comparable performance to MLPs with fewer parameters.

% \subsection{Performance Metrics}

% Figure~\ref{fig:rewards} illustrates the average rewards obtained across the training steps for each environment. In general, the KAN-based PPO matched or exceeded the performance of the MLP-based PPO in most environments. This demonstrates the potential of KANs to achieve robust performance with fewer parameters, particularly in the task HalfCheetah-v4, where the KAN-based models outperformed their MLP counterparts.

% Table~\ref{dmc-scores-table} shows the DMC Proprio scores for the control inputs at 1 million training steps. The KAN-based models performed competitively, sometimes surpassing the MLP configurations in terms of reward mean while maintaining a lower parameter count. This highlights the potential of KANs to provide efficient and effective learning with reduced computational requirements.

% \begin{figure*}[tbp]
%     \centering
%     \includegraphics[width=\linewidth]{images/swimmerok.png}
%     \caption{KAN architecture of Swimmer-v4, illustrating the pruning process to enhance network efficiency.}
%     \label{fig:kan_swimmer}
% \end{figure*}

% \subsection{Discussion}

% The results from our experiments indicate that KANs, when integrated into the PPO framework, can achieve performance comparable to traditional MLPs with significantly fewer parameters. This finding is particularly noteworthy as it demonstrates the efficiency of KANs in reducing the computational complexity of reinforcement learning models without compromising on performance.

% While KAN-based models generally matched or exceeded the performance of MLP-based models, it is important to acknowledge the contexts in which these improvements were observed. For instance, in tasks like HalfCheetah-v4 and Hopper-v4, the KAN-based PPO not only achieved higher rewards but also maintained a lower parameter count, highlighting the efficiency of KANs. However, in some environments like Pusher-v4, the performance improvements were less pronounced, indicating that the benefits of KANs may vary depending on the specific task.

% In our evaluation of 1000 steps on the HalfCheetah-v4 environment, we observed that the MLP with 2 hidden layers of 64 units completed the task significantly faster, with an average elapsed time of 0.37 seconds, compared to the KAN with no hidden layers (k=2, g=3), which took an average of 3.39 seconds. Despite the KAN having far fewer parameters, its increased computational complexity arises from the use of B-splines as activation functions, which require more intricate calculations. The MLP's architecture, while parameter-heavy, benefits from highly optimized implementations in libraries such as Torch, resulting in faster execution times. As KANs are relatively novel, there is a lack of specialized optimization techniques and frameworks designed specifically for them. This discrepancy highlights the potential need for further research and development to enhance the computational efficiency of KANs, making them more viable for real-time applications.

% The lower parameter count in KANs translates to reduced memory usage and potentially faster training times, making them advantageous for deployment in resource-constrained environments. For example, the KAN (k=2, g=3) architecture required significantly fewer parameters compared to the MLP (a=2, c=2) configuration, averaging 348 parameters versus 5348, respectively. This substantial reduction in parameter count underscores the efficiency of KANs in achieving comparable performance with fewer resources.

% An additional aspect to consider is the prune operation depicted in Figure~\ref{fig:kan_swimmer}. Pruning involves reducing the number of parameters in the network by eliminating less important ones, which can further enhance the efficiency and performance of the model. In the context of KANs, pruning can be particularly beneficial due to their already reduced parameter count, allowing for even more streamlined models that maintain high performance. The KAN architecture of Swimmer-v4, as shown in the figure, illustrates this pruning process, which helps optimize the network by focusing on the most critical parameters.

% Additionally, the inherent interpretability of KANs, due to their basis in the Kolmogorov-Arnold representation theorem, provides further benefits for understanding and debugging the learned policies. This interpretability can be crucial in applications where transparency and explainability of the model are important. However, it is crucial to continue exploring and optimizing KAN architectures to fully harness their potential in various reinforcement learning applications.

% In conclusion, the integration of KANs within the PPO framework offers a promising approach to enhancing the efficiency and performance of reinforcement learning models. By achieving comparable performance to MLPs with fewer parameters, KANs present a viable alternative that could lead to more efficient and interpretable reinforcement learning systems.


\section{Results}\label{results}

% The performance of the KAN-based PPO was evaluated against the MLP-based PPO across the selected environments. The primary metrics considered were the average return and the number of parameters. The goal was to assess whether KANs can achieve comparable performance to MLPs with fewer parameters.

The performance of the KAN-based PPO was evaluated against the MLP-based PPO using metrics such as average return and the number of parameters. The average return, defined as the mean cumulative reward over 100 evaluation episodes, provided a robust measure of the policy's effectiveness. The number of parameters, representing the total count of trainable elements in the network, offered insights into the efficiency and potential computational savings achieved by using KANs.

\subsection{Performance Metrics}

Figure~\ref{fig:rewards} illustrates the average rewards obtained across the training steps for each environment. In general, the KAN-based PPO matched or exceeded the performance of the MLP-based PPO in most environments. This demonstrates the potential of KANs to achieve robust performance with fewer parameters, particularly in the task HalfCheetah-v4, where the KAN-based models outperformed their MLP counterparts.

Table~\ref{dmc-scores-table} shows the DMC Proprio scores for the control inputs at 1 million training steps. The KAN-based models performed competitively, sometimes surpassing the MLP configurations in terms of reward mean while maintaining a lower parameter count. This highlights the potential of KANs to provide efficient and effective learning with potentially reduced computational requirements.

\subsection{Discussion}

The results from our experiments indicate that KANs, when integrated into the PPO framework, can achieve performance comparable to traditional MLPs with significantly fewer parameters. This finding is particularly noteworthy as it demonstrates the efficiency of KANs in reducing the computational complexity of reinforcement learning models without compromising on performance. 

While KAN-based models generally matched or exceeded the performance of MLP-based models, it is important to acknowledge the contexts in which these improvements were observed. For instance, in tasks like HalfCheetah-v4 and Hopper-v4, the KAN-based PPO not only achieved higher rewards but also maintained a lower parameter count, highlighting the efficiency of KANs. However, in some environments like Pusher-v4 and Walker2d-v4, the performance improvements were less pronounced, or even worse, indicating that the benefits of KANs may vary depending on the specific task and its complexity. This suggests that maybe adjusting parameters, using a different grid search, or incorporating more neurons might yield better performance in these specific cases.

The lower parameter count in KANs translates to reduced memory usage and potentially faster training times, making them advantageous for deployment in resource-constrained environments. For example, the KAN (k=2, g=3) architecture required significantly fewer parameters compared to the MLP (a=2, c=2) configuration, averaging 348 parameters versus 5348, respectively. This substantial reduction in parameter count underscores the efficiency of KANs in achieving comparable performance with fewer resources.

An additional aspect to consider is the prune operation depicted in Figure~\ref{fig:kan_swimmer}, which involves reducing the number of parameters in the network by eliminating less important ones. Pruning can be particularly beneficial for KANs due to their already reduced parameter count, allowing for even more streamlined models that maintain high performance. The KAN architecture of Swimmer-v4, as shown in the figure, illustrates this pruning process, optimizing the network by focusing on the most critical parameters. Additionally, the inherent interpretability of KANs, based on the Kolmogorov-Arnold representation theorem, provides significant benefits for understanding and debugging the learned policies. This interpretability is crucial in applications where model transparency and explainability are important. However, it is essential to continue exploring and optimizing KAN architectures to fully harness their potential in various reinforcement learning applications.

Despite the efficiency and interpretability benefits, KANs currently face limitations in computational speed. In our evaluation of 1000 steps on the HalfCheetah environment, we observed that the MLP with 2 hidden layers of 64 units completed the task significantly faster, with an average elapsed time of 0.37 seconds, compared to the KAN with no hidden layers (k=2, g=3), which took an average of 3.39 seconds. This increased computational complexity arises from the use of B-splines as activation functions, which require more intricate calculations. The MLP's architecture, while parameter-heavy, benefits from highly optimized implementations in libraries such as Torch, resulting in faster execution times. As KANs are relatively novel, there is a lack of specialized optimization techniques and frameworks designed specifically for them. This discrepancy highlights the potential need for further research and development to enhance the computational efficiency of KANs, making them more viable for real-time applications.

\begin{figure*}[tbp]
     \centering
     \includegraphics[width=\linewidth]{images/Swimmerk2g3.pdf}
     \captionsetup{skip=1pt}
     \caption{KAN architecture of Swimmer-v4, illustrating where the pruning is applied in order to enhance network efficiency.}
     \label{fig:kan_swimmer}
     \vspace{-1mm}
\end{figure*}

==> sections/theoretical.tex <==
\section{Theoretical Background}\label{theoretical}

This section presents the theory and mathematical foundations underpinning our approach.

\subsection{Kolmogorov-Arnold Networks}

Kolmogorov-Arnold Networks leverage the Kolmogorov-Arnold representation theorem, which asserts that any multivariate continuous function can be decomposed into a finite composition of univariate functions and addition operations. Formally, for a smooth function \( f: [0,1]^n \to \mathbb{R} \), this can be expressed as:

\begin{equation}
f(x) = \sum_{q=1}^{2n+1} \Phi_q \left( \sum_{p=1}^{n} \varphi_{q,p}(x_p) \right),
\end{equation}

\noindent where \( \varphi_{q,p}: [0,1] \to \mathbb{R} \) and \( \Phi_q: \mathbb{R} \to \mathbb{R} \) are continuous functions.

In KANs, weight parameters are replaced by learnable 1D functions \( \varphi \), parametrized as B-splines. The computation in a KAN layer with \( n_{\text{in}} \) inputs and \( n_{\text{out}} \) outputs is:

\begin{equation}
x_{l+1,j} = \sum_{i=1}^{n_l} \varphi_{l,j,i}(x_{l,i}),
\end{equation}

\noindent where \( \varphi_{l,j,i} \) is a spline function connecting the \( i \)-th neuron in layer \( l \) to the \( j \)-th neuron in layer \( l+1 \).

The backpropagation process in KANs involves calculating gradients of the spline functions. The loss \( \mathcal{L} \) is minimized using gradient descent, with the gradient of the loss with respect to the spline parameters \( c_i \) computed as:

\begin{equation}
    \frac{\partial \mathcal{L}}{\partial c_i} = \sum_{j=1}^{n_{\text{out}}} \frac{\partial \mathcal{L}}{\partial x_{l+1,j}} \frac{\partial x_{l+1,j}}{\partial c_i},
\end{equation}

\noindent where \( \frac{\partial x_{l+1,j}}{\partial c_i} \) involves the derivative of the spline function with respect to its coefficients.

Comparatively, KANs and MLPs differ as follows:

\begin{itemize}
    \item KANs feature learnable activation functions on edges, while MLPs have fixed activation functions on nodes.
    \item KANs use splines to represent weights, enhancing their capacity to approximate complex functions with fewer parameters.
    \item Both KANs and MLPs can be extended to multiple layers.
\end{itemize}

\subsection{Proximal Policy Optimization}

Proximal Policy Optimization is a policy gradient method that computes an estimator of the policy gradient for use in a stochastic gradient ascent algorithm. The policy gradient estimator is:
\begin{equation}
\hat{g} = \hat{\mathbb{E}}_t \left[ \nabla_\theta \log \pi_\theta(a_t | s_t) \hat{A}_t \right],
\end{equation}
\noindent where \(\pi_\theta\) is the stochastic policy, and \(\hat{A}_t\) is an estimator of the advantage function at timestep \( t \). The expectation \(\hat{\mathbb{E}}_t[ \cdots ]\) denotes the empirical average over a finite batch of samples.

This estimator is derived from the objective function:
\begin{equation}
L_{PG}(\theta) = \hat{\mathbb{E}}_t \left[ \log \pi_\theta(a_t | s_t) \hat{A}_t \right].
\end{equation}

To prevent excessively large policy updates, PPO introduces a clipped surrogate objective. Let \( r_t(\theta) \) denote the probability ratio:
\begin{equation}
r_t(\theta) = \frac{\pi_\theta(a_t | s_t)}{\pi_{\theta_{\text{old}}}(a_t | s_t)}.
\end{equation}

The clipped surrogate objective is defined as:
\begin{equation}
\footnotesize
L_{CLIP}(\theta) = \hat{\mathbb{E}}_t \left[ \min \left( r_t(\theta) \hat{A}_t, \text{clip}(r_t(\theta), 1 - \epsilon, 1 + \epsilon) \hat{A}_t \right) \right],
\end{equation}
\noindent where \(\epsilon\) is a hyperparameter, typically set to 0.2. This objective encourages the new policy to stay within a small region around the old policy by clipping the probability ratio \( r_t(\theta) \) when it exceeds the interval \([1 - \epsilon, 1 + \epsilon]\).

The advantage function \(\hat{A}_t\) can be estimated using Generalized Advantage Estimation (GAE), which reduces variance while introducing a bias controlled by parameter \(\lambda\):
\begin{equation}
\hat{A}_t = \sum_{l=0}^{\infty} (\gamma \lambda)^l \delta_{t+l},
\end{equation}
\noindent where \(\delta_t\) is the temporal difference (TD) error:
\begin{equation}
\delta_t = r_t + \gamma V(s_{t+1}) - V(s_t).
\end{equation}

In practice, PPO uses a combination of the clipped surrogate objective, a value function loss, and an entropy bonus to ensure sufficient exploration. The combined objective function is:
\begin{equation}
\footnotesize
L_{CLIP+VF+S}(\theta) = \hat{\mathbb{E}}_t \left[ L_{CLIP}(\theta) - c_1 L_{VF}(\theta) + c_2 S[\pi_\theta](s_t) \right],
\end{equation}
\noindent where \( L_{VF}(\theta) = (V_\theta(s_t) - V_t^\text{target})^2 \) is the squared-error loss for the value function, \( S[\pi_\theta](s_t) \) is the entropy bonus, and \( c_1, c_2 \) are coefficients.

The PPO technique (Algorithm~\ref{algorithm}) alternates between collecting data through interaction with the environment and optimizing the policy using the clipped surrogate objective.

\begin{algorithm}
\caption{Proximal Policy Optimization}
\label{algorithm}
\begin{algorithmic}[1]
\State Initialize policy parameters \(\theta\)
\For{each iteration}
    \For{actor = 1, 2, ..., N}
        \State Run policy \(\pi_\theta\) in environment for \(T\) timesteps
        \State Compute advantage estimates \(\hat{A}_t\)
    \EndFor
    \State Optimize surrogate \(L_{\text{CLIP}}(\theta)\) with \(K\) epochs and minibatch size \(M \leq NT\)
    \State Update policy parameters \(\theta\)
\EndFor
\end{algorithmic}
\end{algorithm}

